Combined Covers and Beth Definability (Extended Version)

In ESOP 2008, Gulwani and Musuvathi introduced a notion of cover and exploited it to handle infinite-state model checking problems. Motivated by applications to the verification of data-aware processes, we proved in a previous paper that covers are strictly related to model completions, a well-known topic in model theory. In this paper we investigate cover transfer to theory combinations in the disjoint signatures case. We prove that for convex theories, cover algorithms can be transferred to theory combinations under the same hypothesis (equality interpolation property aka strong amalgamation property) needed to transfer quantifier-free interpolation. In the non-convex case, we show by a counterexample that covers may not exist in the combined theories, even in case combined quantifier-free interpolants do exist. However, we exhibit a cover transfer algorithm operating also in the non-convex case for special kinds of theory combinations; these combinations (called `tame combinations') concern multi-sorted theories arising in many model-checking applications (in particular, the ones oriented to verification of data-aware processes).

==> app_example.tex <==
\section{Appendix}\label{app}

In this Appendix we give a detailed pedantic account of the computations required to solve Example~\ref{ex}.

Formula~\eqref{eq:ex0} is already purified.
%se si vuole restaurare la nota aggiungere il letterale che manca
%\footnote{A non-purified problem whose purification is equal to~\eqref{eq:ex0} (up to renaming) is 
%$$
%\exists e\;(x_1+f(x_1) \leq e \;\wedge\; e \leq x_2+f(x_2)\; \wedge\; f(x_2+f(e))=x_1)~~.
%$$
%}
 Notice also that the variables $e_1, e_2$ are in fact already explicitly  defined (only $e_3, e_4$ are truly existential variables). 
 
 We first make the partition guessing. There is no need to involve defined variables into the partition guessing, hence we need to consider only two partitions; they  are described by the following  formulae:
 \begin{eqnarray*}
  E_1(e_3, e_4) ~&\equiv&~ e_3\neq e_4 
  \\
  E_2(e_3, e_4) ~&\equiv&~ e_3= e_4 
 \end{eqnarray*}
We first analyze  \textbf{the case of $E_1$}.  The formulae $\psi_1$ and $\psi_2$ to which we need to apply exhaustively Step (1) and Step (2i) of our algorithm are:
\begin{eqnarray*}
 \psi_1 ~&\equiv&~f(e_3)=e_3\,\wedge\, \; f(e_4)= x_1\;\wedge\; e_3\neq e_4
 \\
 \psi_2 ~&\equiv&~x_1+e_1\leq e_3\;\wedge\; e_3\leq x_2+e_2\;\wedge \;e_4=x_2+e_3\;
 \wedge\; e_3\neq e_4
\end{eqnarray*}
%
 We first compute the implicit definability formulae for the truly existential variables with respect to both $T_1$ and $T_2$.

\begin{description}
 \item[-] We first consider $\mathtt{ImplDef}_{\psi_1,e_3}^{T_1}(\ux,\uz)$.  Here we show that the cover of the negation of formula~\eqref{eq:def} is equivalent to $\top$ (so that $\mathtt{ImplDef}_{\psi_1,e_3}^{T_1}(\ux,\uz)$ is equivalent to $\bot$). We must quantify over truly existential variables and their duplications, thus we need to compute the cover of
 $$
 f(e'_3)=e'_3\wedge f(e_3)=e_3\wedge  f(e'_4)=x_1\wedge f(e_4)=x_1\wedge e_3\neq e_4 \wedge e'_3 \neq e'_4\wedge  e'_3\neq e_3
 $$
  This is a saturated set according to the superposition based procedure of~\cite{cade19}, hence the result is $\top$, as claimed.
 \item[-] The formula $\mathtt{ImplDef}_{\psi_1,e_4}^{T_1}(\ux,\uz)$ is also equivalent to $\bot$, by the same  argument as above.
 \item[-] To compute $\mathtt{ImplDef}_{\psi_2,e_3}^{T_2}(\ux,\uz)$ we  use Fourier-Motzkin quantifier elimination. We need to eliminate the variables $e_3, e'_3, e_4, e'_4$ (intended as existentially quantified variables) from 
 \begin{equation*}
 \begin{aligned}
 &
 x_1+e_1\leq e'_3\leq x_2+e_2\wedge x_1+e_1\leq e_3\leq x_2+e_2\wedge e'_4=x_2+e'_3\wedge
 \\ & \wedge
 e_4=x_2+e_3 \wedge e_3\neq e_4 \wedge e'_3 \neq e'_4\wedge e'_3\neq e_3~~.
 \end{aligned}
 \end{equation*}
 This gives $x_1+e_1\neq x_2+e_2 \wedge x_2\neq 0$, so that $\mathtt{ImplDef}_{\psi_2,e_3}^{T_2}(\ux,\uz)$ is 
 $x_1+e_1= x_2+e_2 \wedge x_2\neq 0$. The corresponding equality interpolating term for $e_3$ is $x_1+e_1$. 
 \item[-] The formula $\mathtt{ImplDef}_{\psi_2,e_4}^{T_2}(\ux,\uz)$ is also equivalent to 
 $x_1+e_1= x_2+e_2\wedge x_2\neq 0$ and the  equality interpolating term for $e_4$ is $x_1+e_1+x_2$.
% this conjunct is inconsitent with $\psi_2$, so Step (2i) would result in an inconsistent formula 
% (on the other hand, adding $\neg\mathtt{ImplDef}_{\psi_2,e_4}^{T_2}(\ux,\uz)$ to $\psi_2$ as in Step 1 does not yield any effect: one would just add an implied literal).
\end{description}
 
So, if we apply Step 1 we get\footnote{The literal $x_2\neq 0$ is entailed by $\psi_2$, so we can simplify it to $\top$ in $\mathtt{ImplDef}_{\psi_2,e_3}^{T_2}(\ux,\uz)$ and $\mathtt{ImplDef}_{\psi_2,e_4}^{T_2}(\ux,\uz)$.}
 \begin{equation}\label{eq:ex1}
 \exists e_1\cdots \exists e_4
 \left( 
\begin{aligned}
&
%e_0=f(f(x_1))\;\wedge \;
e_1= f(x_1)\;\wedge\; e_2=f(x_2)\; \wedge
\\ & \wedge\,
f(e_3)=e_3\,\wedge\, \; f(e_4)= x_1\;\wedge \; e_3\neq e_4\;\wedge
\\ & \wedge\,
 x_1+e_1\leq e_3\,\wedge\, e_3\leq x_2+e_2\,\wedge \, e_4=x_2+e_3
 \, \wedge \, x_1+e_1\neq x_2+e_2
%e_0\leq e_3\;\wedge\; e_3\leq e_1-e_2+e_0\;\wedge \;e_5=x_2+e_4
 \end{aligned}
 \right)
\end{equation}
 If we apply Step
 (2i) (for i=3), we get (after removing implied equalities)
 \begin{equation}\label{eq:ex2}
 \exists e_1\cdots \exists e_4\;
~ \left( 
\begin{aligned}
&
%e_0=f(f(x_1))\;\wedge \;
e_1=f(x_1)\;\wedge\; e_2=f(x_2)\; \wedge\; e_3=x_1+e_1 \;\wedge
\\ & \wedge\,
f(e_3)=e_3\,\wedge\, \; f(e_4)= x_1\;\wedge\; e_3\neq e_4\;\wedge
\\ & \wedge\;
e_4=x_2+e_3 \;\wedge\;
 x_1+e_1= x_2+e_2
%e_1=e_2\;\wedge \;
 \end{aligned}
 \right)
\end{equation}
Step (2i) (for i=4)  gives a formula logically equivalent to~\eqref{eq:ex2}.
Notice that~\eqref{eq:ex2} is terminal too, because all existential variables are now explicitly defined (this is a side-effect of the fact that $e_3$ has been moved to the defined variables).
Thus the exhaustive application of Steps (1) and (2i) is concluded.

Applying the final step of Proposition~\ref{prop:terminal} to~\eqref{eq:ex2} is quite easy: it is sufficient to unravel the acyclic definitions. The result, after little simplification, is
\begin{equation*}
 x_2\neq 0\, \wedge\, x_1+f(x_1)= x_2+f(x_2)\, \wedge\, f(x_2+f(x_1+f(x_1)))=x_1\, \wedge\, f(x_1+f(x_1))= x_1+f(x_1);
\end{equation*}
this can be further simplified to
\begin{equation}\label{eq:res11}
 x_2\neq 0\, \wedge\, x_1+f(x_1)= x_2+f(x_2)\, \wedge\, f(2x_2+f(x_2))=x_1\, \wedge\, f(x_1+f(x_1))= x_1+f(x_1);
\end{equation}


As to formula~\eqref{eq:ex1}, we need to apply  the final cover computations mentioned in Proposition~\ref{prop:terminal}. The formulae $\psi_1$ and $\psi_2$ are now
\begin{eqnarray*}
 \psi'_1~\equiv~
 &
 f(e_3)=e_3\;\wedge\, \; f(e_4)= x_1\;\wedge\, \; e_3\neq e_4~~~~~~~~~~~~~~~~
 \\
 \psi'_2~\equiv~
 &
 x_1+e_1\leq e_3 \leq x_2+e_2\,\wedge \, e_4=x_2+e_3
 \, \wedge \, x_1+e_1\neq x_2+e_2\;\wedge \; e_3\neq e_4
\end{eqnarray*}
The $T_1$-cover of $\psi_1'$ is $\top$. For the $T_2$-cover of $\psi_2'$,  
eliminating, with Fourier-Motzkin the variables $e_4$ and  $e_3$, we get
\begin{equation*}
x_1+e_1< x_2+e_2\,\wedge \,x_2\neq 0
\end{equation*}
which becomes
\begin{equation}\label{eq:res12}
x_1+f(x_1)< x_2+f(x_2)\,\wedge \,x_2\neq 0
\end{equation}
after unravelling the explicit definitions of $e_1, e_2$.
Thus, \emph{the analysis of the case of the partition $E_1$ gives, as a result, the disjunction of~\eqref{eq:res11} and 
~\eqref{eq:res12}.}


We now analyze  \textbf{the case of $E_2$}. Before proceeding, we replace $e_4$ with $e_3$ (since $E_2$ precisely asserts that these two variables coincide); our formulae $\psi_1$ and $\psi_2$ become
\begin{eqnarray*}
 \psi''_1 ~&\equiv&~f(e_3)=e_3\,\wedge\, \; f(e_3)= x_1
 \\
 \psi''_2 ~&\equiv&~x_1+e_1\leq e_3\;\wedge\; e_3\leq x_2+e_2\;\wedge \;0=x_2\;
\end{eqnarray*}
From $\psi''_1$ we deduce $e_3=x_1$, thus we can move $e_3$ to the explicitly defined variables.\footnote{ This avoids useless calculations:  the implicit definability condition for  variables  having an entailed explicit definition is obviously $\top$, so making case split on it produces either tautological consequences or inconsitencies.} In this way we get the terminal working formula 
\begin{equation}\label{eq:ex3}
 \exists e_1\cdots \exists e_3
 \left( 
\begin{aligned}
&
%e_0=f(f(x_1))\;\wedge \;
e_1= f(x_1)\;\wedge\; e_2=f(x_2)\; \wedge \; e_3=x_1
\\ & \wedge\,
f(e_3)=e_3\,\wedge\, \; f(e_3)= x_1\;\wedge \; 
\\ & \wedge\,
 x_1+e_1\leq e_3\,\wedge\, e_3\leq x_2+e_2\,\wedge \, 0=x_2
%e_0\leq e_3\;\wedge\; e_3\leq e_1-e_2+e_0\;\wedge \;e_5=x_2+e_4
 \end{aligned}
 \right)
\end{equation}
Unravelling the expicit definitions, we get (after exhaustive simplifications)
\begin{equation}\label{eq:res2}
 x_2=0 \; \wedge \; f(x_1)=x_1 \;\wedge \; x_1 \leq 0 \; \wedge\; x_1\leq f(0)  
\end{equation}


Now, the disjunction of~\eqref{eq:res11},\eqref{eq:res12} and~\eqref{eq:res2} is precisely the final result~\eqref{eq:res} claimed in Section~\ref{sec:combined}. This concludes our detailed analysis of Example~\ref{ex}.


==> super.tex <==
\section{Strong Amalgamation and Equality Interpolation}\label{sec:strongamalgamation} %AG: questa sezione sono di fatto altri preliminaries...bisognerebbe chiarire meglio le motivation, ossia dire fin dalla prima frase della sezione che questi main results presi da altri lavori sono funzionali per la nostra combined procedures, per dare condizioni necessarie e sufficienti

We report here the main results from~\cite{bgr-acmtocl} and from old  literature like~\cite{amalgam} concerning amalgamation, strong amalgamation and quantifier-free interpolation (some definitions and results are slightly simplified  because we restrict them to the case of universal theories).

\begin{definition}
  \label{def:amalgamation}
  A universal theory $T$ has the \emph{amalgamation property} iff whenever
  we are given models $\cM_1$ and $\cM_2$ of $T$ and a common
  substructure $\cM_0$ of them, there exists a further model $\cM$ of
  $T$ endowed with embeddings $\mu_1:\cM_1 \longrightarrow \cM$ and
  $\mu_2:\cM_2 \longrightarrow \cM$ whose restrictions to $|\cM_0|$
  coincide.\footnote{For the results of this paper to be correct, the
    notion of structure (and of course that of substructure) should
    encompass the case of structures with empty domains.
    %
    Readers feeling uncomfortable with empty domains can assume that
    signatures always contain an individual constant.  }

  A universal theory $T$ has the \emph{strong amalgamation property} if the
  above embeddings $\mu_1, \mu_2$ and the above model $\cM$ can be chosen so to satisfy the following additional
  condition: if for some $m_1, m_2$ we have $\mu_1(m_1)=\mu_2(m_2)$,
  then there exists an element $a$ in $|\cM_0|$ such that $m_1=a=m_2$.
\end{definition}

Amalgamation and strong amalgamation are strictly related to quantifier-free interpolation and to combined quantifier-free interpolation, as the results below show:
\begin{theorem}\cite{amalgam}
  \label{thm:interpolation-amalgamation} 
  A universal theory $T$ has the amalgamation property iff it admits
  quan\-ti\-fier-free interpolants.
\end{theorem}

A theory $T$ is \emph{stably infinite} iff every $T$-satisfiable
constraint is satisfiable in
an infinite model of $T$. 
The following Lemma comes from a trivial compactness argument:
\begin{lemma}\label{lem:si}
 If $T$ is stably infinite, then every finite or countable model $\cM$ of $T$ can be embedded in a model $\cN$ of $T$ such
 that  $\vert \cN\vert \setminus \vert \cM\vert$ is countable.
\end{lemma}
\begin{proof}
 Consider $T\cup\Delta(\cM)\cup \{c_i\neq a\, \mid\, a\in \vert \cM\vert\}_i\cup \{c_i\neq c_j\}_{i\neq j}$, where $\{c_i\}_i$ is a countable set of fresh constants: by the Diagram Lemma and the downward L\"oweneheim-Skolem theorem~\cite{CK}, it is sufficient to show that this set is consistent. Suppose not; then by compactness $T\cup\Delta_0\cup \Delta_1\cup\{c_i\neq c_j\}_{i\neq j}$ is not satisfiable, for a finite subset $\Delta_0$ of $\Delta(\cM)$ and a finite subset $\Delta_1$ of 
 $ \{c_i\neq a\, \mid\, a\in \vert \cM\vert\}_i$. However, this is a contradiction because by stable infiniteness, $\Delta_0$, being satisfiable in $\cM$, is also satisfiable in an infinite model of $T$. 
\end{proof}

%By compactness, it is easily seen  that
%$T$ is {stably infinite} iff every model of $T$ embeds into an
%infinite one (see for instance~\cite{Ghil05}). 
%A theory $T$ is \emph{convex} iff
%Recall that a theory $T$ is \emph{stably infinite} iff every $T$-satisfiable constraint is satisfiable in an infinite model of $T$.

\begin{theorem}\cite{bgr-acmtocl}
 \label{thm:sub-amalgamation_transfer}
 Let $T_1$ and $T_2$ be two universal stably infinite theories over disjoint
 signatures $\Sigma_1$ and $\Sigma_2$.  If both $T_1$ and $T_2$ have
 the strong amalgamation property, then so does $T_1\cup T_2$ (hence, in particular,
 the quantifier-free interpolation property transfers from $T_1$ and $ T_2$ to their combination $T_1\cup T_2$). 
\end{theorem}

There is a converse of the previous result; for a signature $\Sigma$, let us call $\EUF(\Sigma)$ the pure equality theory over the signature $\Sigma$ (this theory is easily seen to have the strong amalgamation property).


\begin{theorem}\cite{bgr-acmtocl}
  \label{prop:strong_amalgamation_needed} 
  Let $T$ be a stably infinite universal theory 
  %admitting quantifier-free interpolation 
  and let
  $\Sigma$ be a signature disjoint from the signature of $T$
  containing at least a unary predicate symbol.  Then, $T\cup
  \EUF(\Sigma)$ has quantifier-free interpolation iff $T$ has the
  strong amalgamation property.
\end{theorem}

According to Theorem~\ref{thm:interpolation-amalgamation}, the amalgamation property has a syntactic counterpart (namely quantifier-free interpolation); there is an analogous syntactic characterization for strong amalgamation~\cite{bgr-acmtocl}, which can be exploited in the design of combined interpolation algorithms~\cite{bgr-acmtocl}. Since such a condition is rather complex, we report it here only for the simplified case of convex theories, where it coincides with a well-known condition previously introduced in~\cite{ym}.
Recall that a theory $T$ is \emph{convex} iff 
for every constraint $\delta$, if $T\vdash\delta \to
\bigvee_{i=1}^n x_i=y_i$ then $T\vdash\delta\to x_i=y_i$ holds for some
$i\in \{1, ..., n\}$.

\begin{definition}
  \label{def:YM}
   A convex universal theory $T$ is \emph{equality interpolating}  iff 
   %it satisfies the following condition: 
   %\begin{itemize}
   %  \item 
     for every pair $y_1, y_2$ of variables and for every pair
       of \emph{constraints} $\delta_1(\ux,\uz_1, y_1),
       \delta_2(\ux,\uz_2,y_2)$ such that
       \begin{equation}
         \label{eq:ym_ant}
         T\vdash\delta_1(\ux, \uz_1,y_1)\wedge
         \delta_2(\ux,\uz_2, y_2)\to
         y_1= y_2
       \end{equation}
       there exists a term $t(\ux)$ such that
       \begin{equation}
         \label{eq:ym_cons}
         T\vdash
         \delta_1(\ux, \uz_1, y_1)\wedge
         \delta_2(\ux, \uz_2, y_2)\to
         y_1= t  \wedge  y_2= t.
       \end{equation}
  % \end{itemize}
\end{definition}


\begin{theorem}\cite{bgr-acmtocl}
  \label{thm:strong_amalgamation_syntactic}
  A convex universal theory $T$ having quan\-ti\-fier-free interpolation
  has the strong amalgamation property iff it is equality interpolating.
\end{theorem}

In conclusion, if $T_1, T_2$ are universal, convex, stably infinite,\footnote{
A convex theory $T$ is `almost' stably infinite in the sense that every constraint which is $T$-satisfiable in a $T$-model whose support has at least two elements is satisfiable also in an infinite $T$-model. The one-element model can be used to build counterexamples, though: e.g.
the theory of Boolean algebras is convex (like any other universal Horn theory) but the constraint $x=0 \wedge x=1$ is only satisfiable in the degenerate one-element Boolean algebra.
} have disjoint signatures and have quantifier-free interpolation, in order for $T_1\cup T_2$ to have quantifier-free interpolation too, we need to ask that both $T_1$ and $T_2$ are equality interpolating; in view of Theorem~\ref{prop:strong_amalgamation_needed}, this condition is not only sufficient but also (almost) necessary.

In~\cite{bgr-acmtocl} a long list of universal strongly amalgamable (i.e. both quantifier-free interpolating and equality interpolating) theories is given, comprising both convex and non-convex theories. The list includes $\EUF(\Sigma)$, recursive data theories, as well as linear (both integer  and real) arithmetics. For linear arithmetics (and fragments of its), it is essential to make a very careful choice of the signature, see again~\cite{bgr-acmtocl} (especially Subsection 4.1) for details.  All the above theories admit a model completion (which coincides with the theory itself in case the theory admits quantifier elimination).

The equality interpolating property in a convex theory $T$ can be equivalently characterized using Beth definability as follows. Consider a primitive formula $\exists \uz \phi(\ux, \uz,y)$ (here $\phi$ is a conjunction of literals); we say that
$\exists \uz\, \phi(\ux, \uz,y)$ \emph{implicitly defines $y$} in $T$ iff the following formula
\begin{equation}\label{eq:bethimpl}
 \forall y \,\forall y'\;( \exists \uz \phi(\ux, \uz,y)\wedge \exists \uz \phi(\ux, \uz,y') \to y= y')
\end{equation}
is $T$-valid.
We say that $\exists \uz \phi(\ux, \uz,y)$ \emph{explicitly defines $y$} in $T$ iff there is a term $t(\ux)$ such that the formula
\begin{equation}\label{eq:bethexpl}
 \forall y \;( \exists \uz \phi(\ux, \uz,y) \to y= t(\ux))
\end{equation}
 is $T$-valid.

 For future use, we notice that,
  by trivial logical manipulations, the formulae~\eqref{eq:bethimpl} and~\eqref{eq:bethexpl} are logically equivalent to
\begin{equation}\label{eq:bethimpl1}
  \forall y\forall \uz \forall y'\forall \uz'( \phi(\ux, \uz,y)\wedge \phi(\ux, \uz',y') \to y= y')~~~.
\end{equation}
and to
\begin{equation}\label{eq:bethexpl1}
 \forall y \forall \uz (\phi(\ux, \uz,y) \to y= t(\ux))
\end{equation}
respectively (we shall use such equivalences without explicit mention).

We say that a theory $T$ has the \emph{Beth definability property for primitive formulae} iff whenever a primitive formula
$\exists \uz\, \phi(\ux, \uz,y)$ implicitly defines  the variable $y$ then it also explicitly defines it.

\begin{theorem}\cite{bgr-acmtocl}
  \label{thm:beth}
  A convex theory $T$ having quan\-ti\-fier-free interpolation
   is equality interpolating iff it has the Beth definability property for primitive formulae.
\end{theorem}

\begin{proof}
 We recall the easy proof of the left-to-right side (this is the only side we need in this paper). Suppose that $T$ is equality interpolating and that  
 \begin{equation*}
 T\vdash \phi(\ux, \uz,y)\wedge \phi(\ux, \uz',y') \to y= y'~~;
\end{equation*}
then there is a term $t(\ux)$ such that
\begin{equation*}
 T\vdash \phi(\ux, \uz,y)\wedge \phi(\ux, \uz',y') \to y=t(\ux) \wedge  y'=t(\ux)~~.
\end{equation*}
Replacing $\uz',y'$ by $\uz,y$ via a substitution, we get precisely~\eqref{eq:bethexpl1}. %AG: Prima era: 'Replacing $\uz',y$ by $\uz,y$ via a substitution,' il primo y dovrebbe essere y'.
\end{proof}

